Forensic Iris Image-Based Post-Mortem Interval Estimation

Post-mortem iris recognition is an emerging application of iris-based human identification in a forensic setup. One factor that may be useful in conditioning iris recognition methods is the tissue decomposition level, which is correlated with the post-mortem interval (PMI), \ie the number of hours that have elapsed since death. PMI, however, is not always available, and its precise estimation remains one of the core challenges in forensic examination. This paper presents the first known to us method of the PMI estimation directly from iris images captured after death. To assess the feasibility of the iris-based PMI estimation, we designed models predicting the PMI from (a) near-infrared (NIR), (b) visible (RGB), and (c) multispectral (RGB+NIR) forensic iris images. Models were evaluated following a 10-fold cross-validation, in (S1) sample-disjoint, (S2) subject-disjoint, and (S3) cross-dataset scenarios. We explore two data balancing techniques for S3: resampling-based balancing (S3-real), and synthetic data-supplemented balancing (S3-synthetic). We found that using the multispectral data offers a spectacularly low mean absolute error (MAE) of $\approx 3.5$ hours in the scenario (S1), a bit worse MAE $\approx 17.5$ hours in the scenario (S2), and MAE $\approx 45.77$ hours in the scenario (S3). Additionally, supplementing the training set with synthetically-generated forensic iris images (S3-synthetic) significantly enhances the models' ability to generalize to new NIR, RGB and multispectral data collected in a different lab. This suggests that if the environmental conditions are favorable (\eg, bodies are kept in low temperatures), forensic iris images provide features that are indicative of the PMI and can be automatically estimated.

==> figure_tex/nij_multispectral_plot.tex <==
\begin{figure*}[ht] 
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_multispectral_vgg.pdf}
        \caption{VGG19}
        \label{nij-multispectral:vgg19}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_multispectral_inception.pdf}
        \caption{Inception\_v3}
        \label{nij-multispectral:inception}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_multispectral_densenet.pdf}
        \caption{DenseNet121}
        \label{nij-multispectral:densenet121}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_multispectral_resnet.pdf}
        \caption{ResNet152}
        \label{nij-multispectral:resnet152}
    \end{subfigure}
    \caption{Scatter plots visualizing the predicted PMI values against the actual PMI values for \textbf{multispectral data} by models trained on the Warsaw dataset and \textbf{tested on the NIJ dataset}.}%Scatter plots visualize the PMI estimation performance of each model trained on \textbf{multispectral data} of the Warsaw dataset and \textbf{tested on the NIJ dataset}, depicting the predicted PMI values against the actual PMI values.}
    \label{fig:nij_multispectral_model_plot} 
\end{figure*} 


==> figure_tex/nij_nir_plot.tex <==
\begin{figure*}[ht] 
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_nir_vgg.pdf}
        \caption{VGG19}
        \label{nij-nir:vgg19}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_nir_inception.pdf}
        \caption{Inception\_v3}
        \label{nij-nir:inception}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_nir_densenet.pdf}
        \caption{DenseNet121}
        \label{nij-nir:densenet121}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_nir_resnet.pdf}
        \caption{ResNet152}
        \label{nijnir:resnet152}
    \end{subfigure}
    \caption{Scatter plots visualizing the predicted PMI values against the actual PMI values for \textbf{NIR data} by models trained on the Warsaw dataset and \textbf{tested on the NIJ dataset}.}%Scatter plots visualize the PMI estimation performance of each model trained on \textbf{NIR data} of the Warsaw dataset and \textbf{tested on the NIJ dataset}, depicting the predicted PMI values against the actual PMI values.}
    \label{fig:nij_nir_model_plot} 
\end{figure*} 


==> figure_tex/nij_rgb_plot.tex <==
\begin{figure*}[ht] 
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_rgb_vgg.pdf}
        \caption{VGG19}
        \label{nij-rgb:vgg19}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_rgb_inception.pdf}
        \caption{Inception\_v3}
        \label{nij-rgb:inception}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_rgb_densenet.pdf}
        \caption{DenseNet121}
        \label{nij-rgb:densenet121}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nij_rgb_resnet.pdf}
        \caption{ResNet152}
        \label{nij-rgb:resnet152}
    \end{subfigure}
    \caption{Scatter plots visualizing the predicted PMI values against the actual PMI values for \textbf{RGB data} by models trained on the Warsaw dataset and \textbf{tested on the NIJ dataset}.}%Scatter plots visualize the PMI estimation performance of each model trained on \textbf{RGB data} of the Warsaw dataset and \textbf{tested on the NIJ dataset}, depicting the predicted PMI values against the actual PMI values.}
    \label{fig:nij_rgb_model_plot} 
\end{figure*} 


==> figure_tex/warsaw_multispectral_plot.tex <==
\begin{figure*}[ht] 
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_multispectral_vgg.pdf}
        \caption{VGG19}
        \label{warsaw-multispectral:vgg19}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_multispectral_inception.pdf}
        \caption{Inception\_v3}
        \label{warsaw-multispectral:inception}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_multispectral_densenet.pdf}
        \caption{DenseNet121}
        \label{warsaw-multispectral:densenet121}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_multispectral_resnet.pdf}
        \caption{ResNet152}
        \label{warsaw-multispectral:resnet152}
    \end{subfigure}
    \caption{Scatter plots visualizing the predicted PMI values against the actual PMI values for \textbf{multispectral data} by models trained on the NIJ dataset and \textbf{tested on the Warsaw dataset}.}%Scatter plots visualize the PMI estimation performance of each model trained on \textbf{multispectral data} of the NIJ dataset and \textbf{tested on the Warsaw dataset}, depicting the predicted PMI values against the actual PMI values.}
    \label{fig:warsaw_multispectral_model_plot} 
\end{figure*} 


==> figure_tex/warsaw_nir_plot.tex <==
\begin{figure*}[ht] 
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_nir_vgg.pdf}
        \caption{VGG19}
        \label{warsaw-nir:vgg19}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_nir_inception.pdf}
        \caption{Inception\_v3}
        \label{warsaw-nir:inception}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_nir_densenet.pdf}
        \caption{DenseNet121}
        \label{warsaw-nir:densenet121}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_nir_resnet.pdf}
        \caption{ResNet152}
        \label{warsawnir:resnet152}
    \end{subfigure}
    \caption{Scatter plots visualizing the predicted PMI values against the actual PMI values for \textbf{NIR data} by models trained on the NIJ dataset and \textbf{tested on the Warsaw dataset}.}
    \label{fig:warsaw_nir_model_plot} 
\end{figure*} 

==> figure_tex/warsaw_rgb_plot.tex <==
\begin{figure*}[ht] 
    \centering
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_rgb_vgg.pdf}
        \caption{VGG19}
        \label{warsaw-rgb:vgg19}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_rgb_inception.pdf}
        \caption{Inception\_v3}
        \label{warsaw-rgb:inception}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_rgb_densenet.pdf}
        \caption{DenseNet121}
        \label{warsaw-rgb:densenet121}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/warsaw_rgb_resnet.pdf}
        \caption{ResNet152}
        \label{warsaw-rgb:resnet152}
    \end{subfigure}
    \caption{Scatter plots visualizing the predicted PMI values against the actual PMI values for \textbf{RGB data} by models trained on the NIJ dataset and \textbf{tested on the Warsaw dataset}.}%Scatter plots visualize the PMI estimation performance of each model trained on \textbf{RGB data} of the NIJ dataset and \textbf{tested on the Warsaw dataset}, depicting the predicted PMI values against the actual PMI values.}
    \label{fig:warsaw_rgb_model_plot} 
\end{figure*} 


==> table_tex/multispectral_testset_nij.tex <==
\begin{table}[ht]
\centering
\caption{Same as in Tab. \ref{tab:nir-testset-nij} for \textbf{multispectral data}.}
\vspace{-0.3cm}
\label{tab:multispectral-testset-nij}
\begin{tabular}{lcccc}
%\toprule \toprule
 & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{MAE} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Model \\ Backbone\end{tabular}} & Mean & StDev & Mean & StDev \\ \midrule
% AlexNet &197.78 &3.25 & 77.19 &1.72 \\
VGG19 &152.56 &3.49 &85.46 &6.14 \\
Inception\_v3 &152.82 &4.19 &81.32 &5.52 \\
\textbf{DenseNet121} &\textbf{136.00} &\textbf{4.46} &\textbf{68.55} &\textbf{0.73} \\
ResNet152 &152.63 &3.36 &77.66 &3.90 \\
%\bottomrule
\end{tabular}
\end{table}


==> table_tex/multispectral_testset_warsaw.tex <==
\begin{table}[ht]
\centering
\caption{Same as in Tab. \ref{tab:nir-testset-warsaw} for \textbf{multispectral data}.}
\label{tab:multispectral-testset-warsaw}
\vskip1mm
\begin{tabular}{lcccc}
%\toprule \toprule
 & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{MAE} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Model \\ Backbone\end{tabular}} & Mean & StDev & Mean & StDev \\ \midrule
% \textbf{AlexNet} &\textbf{109.42} &\textbf{2.05} & \textbf{65.21} &\textbf{1.48} \\
VGG19 &107.68 &5.44 &69.58 &2.64 \\
Inception\_v3 &109.82 &3.62 &69.22 &0.83 \\
DenseNet121 &112.74 &2.50 &70.04 &1.36 \\
\textbf{ResNet152} &\textbf{111.31} &\textbf{6.49} &\textbf{69.12} &\textbf{2.16} \\
%\bottomrule
\end{tabular}
\end{table}


==> table_tex/nir_testset_nij.tex <==
\begin{table}[ht]
\centering
\caption{PMI (in hours) estimated on the \textbf{NIR data} by models trained on Warsaw dataset and \textbf{tested on NIJ} dataset.}
\vspace{-0.3cm}
\label{tab:nir-testset-nij}
\vskip1mm
\begin{tabular}{lcccc}
%\toprule \toprule
 & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{MAE} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Model \\ Backbone\end{tabular}} & Mean & StDev & Mean & StDev \\ \midrule
% AlexNet &208.43 &6.87 & 78.97 &3.01 \\
VGG19 &165.37 &4.39 &76.67 &0.98 \\
Inception\_v3 &170.66 &6.26 &80.83 &2.80 \\
DenseNet121 &171.38 &2.43 &77.82 &0.81 \\
\textbf{ResNet152} &\textbf{163.27} &\textbf{6.19} &\textbf{76.36} &\textbf{1.37} \\
%\bottomrule
\end{tabular}
\end{table}


==> table_tex/nir_testset_warsaw.tex <==
\begin{table}[ht]
\centering
\caption{PMI (in hours) estimated on the \textbf{NIR data} by models trained on NIJ dataset and \textbf{tested on Warsaw} dataset.}
\vspace{-0.3cm}
\label{tab:nir-testset-warsaw}
\vskip1mm
\begin{tabular}{lcccc}
%\toprule \toprule
 & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{MAE} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Model \\ Backbone\end{tabular}} & Mean & StDev & Mean & StDev \\ \midrule
% AlexNet &119.09 &2.25 & 72.84 &1.51 \\
VGG19 &112.71 &2.61 &73.14 &1.58 \\
Inception\_v3 &118.18 &3.02 &78.76 &2.07 \\
DenseNet121 &112.20 &2.08 &72.36 &1.46 \\
\textbf{ResNet152} &\textbf{105.62} &\textbf{3.04} &\textbf{71.48} &\textbf{1.15} \\
%\bottomrule
\end{tabular}
\end{table}


==> table_tex/rgb_testset_nij.tex <==
\begin{table}[ht]
\centering
\caption{Same as in Tab. \ref{tab:nir-testset-nij} for \textbf{RGB data}.}
\vspace{-0.3cm}
\label{tab:rgb-testset-nij}
\vskip1mm
\begin{tabular}{lcccc}
%\toprule \toprule
 & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{MAE} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Model \\ Backbone\end{tabular}} & Mean & StDev & Mean & StDev \\ \midrule
% AlexNet &191.53 &4.25 & 78.56 &2.98 \\
VGG19 &98.34 &2.97 &80.59 &1.87 \\
Inception\_v3 &97.34 &3.04 &81.10 &3.39 \\
\textbf{DenseNet121} &\textbf{95.24} &\textbf{2.93} &\textbf{76.32} &\textbf{1.31} \\
ResNet152 &95.31 &4.26 &80.11 &2.67 \\
%\bottomrule
\end{tabular}
\end{table}


==> table_tex/rgb_testset_warsaw.tex <==
\begin{table}[ht]
\centering
\caption{Same as in Tab. \ref{tab:nir-testset-warsaw} for \textbf{RGB data}.}
\vspace{-0.3cm}
\label{tab:rgb-testset-warsaw}
\vskip1mm
\begin{tabular}{lcccc}
%\toprule \toprule
 & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{MAE} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Model \\ Backbone\end{tabular}} & Mean & StDev & Mean & StDev \\ \midrule
% AlexNet &141.05 &3.41 &83.01 &1.83 \\
VGG19 &106.07 &2.79 &88.58 &1.99 \\
\textbf{Inception\_v3} &\textbf{90.14} &\textbf{2.78} &\textbf{73.23} &\textbf{2.05} \\
DenseNet121 &99.68 &1.59 &82.32 &1.07 \\
ResNet152 &98.18 &2.26 &81.15 &2.27 \\
%\bottomrule
\end{tabular}
\end{table}

